Defending against Adaptive Prompt Injection Attacks via Reasoning-enabled Task Alignment

Indirect prompt injection attacks hijack LLM-based agents by embedding malicious instructions in third-party data that the agent retrieves during task execution. Existing defenses report near-zero attack success rate on static benchmarks, yet recent adaptive evaluations show that these results collapse once the attacker is allowed to optimize against the deployed defense. In this work, we trace this collapse to two failure modes. First, existing defense methods are confined to recognizing specific attack patterns, rather than assessing whether the intent of every embedded instruction is relevant to the user task. Second, training-based defenses, which otherwise offer the strongest safety-utility trade-off, assemble their adversarial examples from a handful of hand-crafted templates, and the resulting defender fails to generalize outside that narrow strategy distribution. To address these gaps, we propose RETA, a training-based method that grounds defense decisions on the user tasks rather than attacker-controlled data. At each tool-output step, the defender undertakes chain-of-thought reasoning verifying that its actions are consistent with the user task. Leveraging red-teaming, a simulated attacker synthesizes adversarial training data and receives a dictionary-learning diversity reward, achieving broad coverage of injection-reformulation strategies. Together, these allow the defender to be optimized via multi-objective reinforcement learning and achieve better safety-utility trade-off. Across six black-box adaptive attacks, RETA keeps every per-attack ASR below 10%, with average ASR of 2.92% and 3.75% on the two target models, while preserving most utility under attack and on clean inputs.

==> sections/06_analysis.tex <==
% \section{Analysis}

% \subsection{Pattern-Based Defenses Under Adaptive Attack}

% \subsection{Properties of the Diversity Reward}

% \subsection{Game-Theoretic Interpretation}

==> tables/adv_training_asr.tex <==
\begin{table}[!h]
    \caption{ASR/UA on AgentDojo before and after adversarial training of \qwen. Robustness (\hyperref[req:r1]{R1}) expects lower ASR; utility-under-attack (\hyperref[req:r2]{R2}) expects higher UA.}
    \centering
    \setlength{\tabcolsep}{3pt}
    \def\arraystretch{1.2}
    \begin{tabularx}{\columnwidth}{l|CC}
        \toprule
        \textbf{Attack} & \textbf{ASR$\downarrow$} & \textbf{UA$\uparrow$} \\
        \midrule
        \multicolumn{3}{c}{Attacks used in Training}\\
        \midrule
        \textsc{Direct} & 6.19\% & 57.9\%\\
        \textsc{SuperDirect} & 6.67\% & 56.4\%\\
        \textsc{SystemMsgs.} & 7.14\% & 56.4\%\\
        \textsc{EscapeChar.} & 7.86\% & 56.2\%\\
        \textsc{FakeComp.} & 11.2\% & 54.8\%\\
        \textsc{Combined.} & 17.4\% & 52.1\%\\
        \textsc{RL-Hammer} & 44.8\% & 17.6\%\\
        \midrule
        \multicolumn{3}{c}{Before Adversarial Training}\\
        \midrule
        \textsc{IgnorePrev.} & 25.2\% & 46.0\%\\
        \textsc{InjecAgent} & 25.7\% & 46.0\%\\
        \textsc{ImportantMsgs.} & 27.4\% & 50.5\%\\
        \textsc{ToolKnow.} & 41.9\% & 48.1\%\\
        \textsc{ChatInject.} & 46.2\% & 31.9\%\\
        \midrule
        \textsc{Average} & 33.3\% & 44.5\%\\
        \midrule
        \multicolumn{3}{c}{After Adversarial Training}\\
        \midrule
        \textsc{IgnorePrev.} & 18.1\% & 41.7\%\\
        \textsc{InjecAgent} & 30.7\% & 35.0\%\\
        \textsc{ImportantMsgs.} & 10.7\% & 47.4\%\\
        \textsc{ToolKnow.} & 11.0\% & 50.5\%\\
        \textsc{ChatInject.} & 27.6\% & 29.5\%\\
        \midrule
        \textsc{Average} & 19.6\% & 40.8\%\\
        \bottomrule
    \end{tabularx}
    \label{tab:adv_training_asr}
\end{table}


==> tables/static_vs_adaptive.tex <==
\begin{table}[!h]
    \caption{Highest static vs. adaptive ASR on AgentDojo across baseline defenses, with the per-defense gap $\Delta$. Robustness (\hyperref[req:r1]{R1}) expects lower ASR; the gap shows why static ASR alone is insufficient.}
    \centering
    \setlength{\tabcolsep}{3pt}
    \def\arraystretch{1.2}
    \begin{tabularx}{\columnwidth}{l|C|CC|C}
        \toprule
        \textbf{Attack $\rightarrow$} & \textsc{None} & \textbf{Static} & \textbf{Adaptive} & \textbf{Gap $\Delta$}\\
        \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
        \textbf{Defense $\downarrow$} & \textbf{BU$\uparrow$} & \textbf{ASR$\downarrow$} & \textbf{ASR$\downarrow$} & \textbf{\%$\downarrow$}\\
        \midrule
        \multicolumn{5}{c}{\qwen}\\
        \midrule
        \textbf{Qwen3-4B} & 61.9\% & 46.2\% & 57.5\% & \worseup{11.3\%}\\
        \textbf{Spotlighting} & 57.7\% & 45.7\% & 52.5\% & \worseup{6.79\%}\\
        \textbf{Sandwiching} & 60.8\% & 25.5\% & 27.5\% & \worseup{2.02\%}\\
        \textbf{PromptGuard} & 63.9\% & 31.2\% & 57.5\% & \worseup{26.3\%}\\
        \textbf{PIGuard} & 63.9\% & 5.71\% & 50.0\% & \worseup{44.3\%}\\
        \textbf{DataSentinel} & 57.7\% & 33.6\% & 50.0\% & \worseup{16.4\%}\\
        \textbf{MELON} & 54.6\% & 5.95\% & 30.0\% & \worseup{24.0\%}\\
        \textbf{MetaSecAlign} & 64.9\% & 4.52\% & 25.0\% & \worseup{20.5\%}\\
        \midrule
        \multicolumn{5}{c}{\llama}\\
        \midrule
        \textbf{Llama-3.1-8B} & 48.5\% & 30.5\% & 35.0\% & \worseup{4.52\%}\\
        \textbf{Spotlighting} & 44.3\% & 19.3\% & 20.0\% & \worseup{0.714\%}\\
        \textbf{Sandwiching} & 46.4\% & 10.0\% & 10.0\% & \nochange\\
        \textbf{PromptGuard} & 42.3\% & 15.7\% & 25.0\% & \worseup{9.29\%}\\
        \textbf{PIGuard} & 45.4\% & 3.10\% & 35.0\% & \worseup{31.9\%}\\
        \textbf{DataSentinel} & 44.3\% & 23.1\% & 25.0\% & \worseup{1.90\%}\\
        \textbf{MELON} & 43.3\% & 6.43\% & 32.5\% & \worseup{26.1\%}\\
        \textbf{MetaSecAlign} & 46.4\% & 9.29\% & 20.0\% & \worseup{10.7\%}\\
        \bottomrule
    \end{tabularx}
    \label{tab:static_vs_adaptive}
\end{table}

